Piecewise Stochastic Barrier Functions

This paper presents a novel stochastic barrier function (SBF) framework for safety analysis of stochastic systems based on piecewise (PW) functions. We first outline a general formulation of PW-SBFs. Then, we focus on PW-Constant (PWC) SBFs and show how their simplicity yields computational advantages for general stochastic systems. Specifically, we prove that synthesis of PWC-SBFs reduces to a minimax optimization problem. Then, we introduce three efficient algorithms to solve this problem, each offering distinct advantages and disadvantages. The first algorithm is based on dual linear programming (LP), which provides an exact solution to the minimax optimization problem. The second is a more scalable algorithm based on iterative counter-example guided synthesis, which involves solving two smaller LPs. The third algorithm solves the minimax problem using gradient descent, which admits even better scalability. We provide an extensive evaluation of these methods on various case studies, including neural network dynamic models, nonlinear switched systems, and high-dimensional linear systems. Our benchmarks demonstrate that PWC-SBFs outperform state-of-the-art methods, namely sum-of-squares and neural barrier functions, and can scale to eight dimensional systems.

==> Automatica/Sections/tablesBackup.tex <==

% \vspace{-2mm}
\begin{table*}[t]
\caption{Benchmark results for the \emph{piecewise constant} and \emph{continuous} SBF methods. The three PWC-SBF synthesis methods are:  dual LP, \gls{cegs} and \gls{gd}. These are compared against state-of-the-art methods: \gls{sos} and \gls{nbf}. 
$K$ denotes the size of partition of $X_\safe$, 
$\tau_{p}$ is the computation time for the bounds on the transition kernel,
$\low{P}_\safe$ is the obtained lower bound on the safety probability for $N=10$ time steps,
$\tau_o$ is the computation time for the SBF synthesis,
and \textrm{Deg} is the degree of the \gls{sos} polynomial for SBF.
% and $\tau_o$ are the computation times for the bounds on the transition kernel and synthesize of SBFs, respectively. 
% For each experiment, the total optimization time is settled at a maximum of $10^4 s$, and timed-out otherwise.
% $\low{P}_\safe$
 % $N=10$  number of time-steps. The lower bound on the probability of safety is denoted as $P_\safe$. 
% \LL{Are results for the linear 2 D convex case correct for GD? I guess we need to re-run them until the convergence criteria is met? }
}
\label{table:results}
% \vspace{1mm}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{@{}c|c c| cc | cc | cc | ccc| cc 
!{\color{white}\vline} @{}}
\toprule
 &  &  &   \multicolumn{5}{c }{\hspace{6mm} \underline{Piecewise Constant Stochastic Barriers}} 
  &  &    \multicolumn{4}{c }{\hspace{10mm}\underline{Continuous Stochastic Barriers$^{*}$}} \\
 & & & \multicolumn{2}{c|}{Dual LP} & \multicolumn{2}{c|}{CEGS} &  \multicolumn{2}{c|}{GD} &   \multicolumn{3}{c|}{SOS} &  \multicolumn{2}{c}{NBF}\\
 \cline{2-14}
  {Model}   & {$K$} & $\tau_{p} (s) $  & $\low{P}_\safe$ &$\tau_{0}(s)$ 
   & $\low{P}_\safe$   & $\tau_{o} (s) $ & $\low{P}_\safe$   & $\tau_{o} (s) $ & \textrm{Deg} & $\low{P}_\safe$ & $\tau_{o} (s) $ & $\low{P}_\safe$ & $\tau_{o} (s)$\\
  \hline 
  {Linear}  &  64 & 0.02  & 0.992 &  0.52
 &   0.992   &  0.04 &  0.952 &   0.04    &4 &  0.582 & 0.014  & 0.585 & 3850.93\\
 2D &    225 & 0.31  & 0.998   & 164.60  &  0.998 &   0.44  & 0.973  & 0.20  &  8& 0.582 & 0.265 & 0.940 & 3991.47 
 \\ 
  \textit{Convex }&  900  &  8.85 & 0.999 & 1087.78    & 0.999   & 17.93  & 0.990  & 7.22 & 30  & 0.978  & 151.16  & 0.961& 4025.67\\
  &  2500  &   41.44  & 0.999  & 2897.77  & 0.999   & 88.45   & 0.998   & 52.78  & 36 
   & 0.992  &    458.21 & 0.976 & 4085.65\\
\cline{3-14}
  \hline 
  {Linear}   & 900 & 5.04   & 0.494  & 1197.99 
 &  0.494 &    3.79    & 0.494  &    3.52 &12  & 0.010  & 0.02 & 0.792 & 3546.69
 \\
 2D  & 1225  & 8.20 & 0.800  & 1389.78  & 0.800   & 7.22 & 0.800 & 6.64  & 20 & 0.010 & 11.08 &0.844 & 3579.58
\\ 
 \textit{ Non-Convex}  & 1444 & 9.18  &  0.921 & 1545.45 &  0.921  & 11.65  & 0.921  & 10.12  & 24 & 0.023   & 37.89    & 0.855 & 3589.13
  \\
  & 2926 & 47.98  & 0.927  & 3161.56  & 0.927 &  98.36 & 0.927  &  20.86  & 26 & 0.034   & 62.88 &0.928 &3599.85 
  \\
  & 5890 &  179.94  & 0.929  & 8191.65  &  0.929 & 458.44   &  0.929  & 133.84   & 30 &  0.075 & 196.85 & 0.929&3675.77 \\
     & 11818 & 477.45  & -  & \texttt{TO}  & 0.936  & 1875.49   & 0.936  & 842.67    & 34 & - & \texttt{OM}  & 0.931&3744.23 
     \\
         & 24336 &  987.65  & - & \texttt{TO}  &  0.938  & 4441.55   & 0.938   & 3099.30  & 36 & - &\texttt{OM}  & 0.936 & 4234.56  
        \\
\cline{3-14}
 \hline
{Pendulum}  & 120 & 6.37 & 1.00 & 0.51  &  0.99  & 5.84  & 0.989  & 3.75 & 4  & 0.999 & 7.71  & 0.999 & 4242.89 \\
2D  &    240 & 18.33 &  1.00 & 6.08 & 1.00    & 14.88 & 0.990 & 9.99 & 4 & 0.999 & 34.96 & 0.999 & 4457.82 \\
 &    480 &  37.84  & 1.00 &29.39   &  1.00  &43.42  & 0.999  & 17.88  & 4 & 0.999 & 187.60 & 0.999 & 4675.12
 \\ \cline{3-14}
  \hline
  {Unicycle}  &  1250 & 1103.42 &  0.750 &  1000.19  &  0.750 & 26.37  & 0.750 & 5.68 & 2  & 0.00  & 3110.21   & \cellcolor{gray!25} & \cellcolor{gray!25}  \\
 4D &   1800 & 1756.25  & 0.975  & 1719.58  & 0.975   & 92.26  & 0.975  & 25.78  & 4 & 0.00  &   5451.19  & \cellcolor{gray!25} & \cellcolor{gray!25}  \\
 &  2400 & 2001.11 & 0.998 &  2548.56  & 0.998  & 145.45  &0.998 & 55.59 & 6  & - & \texttt{OM} & \cellcolor{gray!25} & \cellcolor{gray!25} \\
  \hline
   Quadrotor  &  7865 & 80.80  &0.770  & 9906.67 & 0.770 & 1174.49 & 0.770   & 2589.56 &  2  & 0.584  & 0.20  & \cellcolor{gray!25} & \cellcolor{gray!25} 
   \\ 
6D &  15625  & 160.61 & - &\texttt{TO}  & 0.901  & 3788.98& 0.901  & 3258.87 &  8  & 0.900 & 8628.58 & \cellcolor{gray!25} & \cellcolor{gray!25}
   \\ 
   \textit{Convex} &    46656  & 458.59 & - & \texttt{TO}  & -& \texttt{TO}& 0.912   & 9542.75  & 12  &-&\texttt{OM} & \cellcolor{gray!25} & \cellcolor{gray!25} \\  
  \hline
   Quadrotor  &  15625&  188.10  & -&\texttt{TO} & 0.670 & 3845.25   & 0.670 & 3478.31   &  4  & 0.00  & 4.91 & \cellcolor{gray!25} & \cellcolor{gray!25}  \\ 
     6D &    31250& 395.59 & -&\texttt{TO} & 0.810 & 9548.78 & 0.810 & 5878.28 &  8 & 0.00  & 8715.54  & \cellcolor{gray!25} & \cellcolor{gray!25} \\ 
  \textit{Non-Convex} &   46656  & 506.99  &  - & \texttt{TO} &-&\texttt{TO} & 0.900  & 9789.54  & 12  & -& \texttt{OM} & \cellcolor{gray!25} & \cellcolor{gray!25} 
  \\  \hline
   Quadrotor  & 65536  & 845.44  &  - & \texttt{TO}& -& \texttt{TO} & 0.500  & 19377.90 & 2 & 0.00  & 14830.23 &\cellcolor{gray!25} & \cellcolor{gray!25}  \\ 
    8D & 128000 & 2530.74  & -& \texttt{TO} & - & \texttt{TO} &  0.560 & 39132.59  & 4   & - & \texttt{OM} & \cellcolor{gray!25} & \cellcolor{gray!25} \\ 
% \bottomrulermlogit
\bottomrule

\end{tabular}
%% ends scaling the table
}
\text{$^{*}$ For linear systems that use \gls{sos} optimization, the state space is not partitioned. Further, synthesis methods for \gls{sos} and }
\text{ \hspace{0.5mm} \gls{nbf} do not use bounds on the transition kernel.
\ml{Swap SOS and NBF columns?}
}
\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \vspace{-2mm}
% \begin{table*}[t]
\begin{sidewaystable*}[t]
\caption{ This table provides extensive results pertaining \texttt{TO}the case studies for safety verification based on \emph{piecewise constant} and \emph{continuous} stochastic barriers, as briefly established 
in Table~\ref{table:results}.
}
\label{table:results_full}
% \vspace{1mm}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{@{}c| c c| ccc | cccc | cccc || ccccc | cccc
!{\color{white}\vline}
@{}}
\toprule
 &      \multicolumn{15}{c }{\underline{Piecewise Constant Stochastic Barriers}} 
 &  \multicolumn{5}{c }{\underline{Continuous Stochastic Barriers}} 
 \\
 &     & &  \multicolumn{3}{c}{ Dual Linear Program}  & \multicolumn{4}{c }{Counter-Example Guided} & \multicolumn{4}{c||}{Gradient Descent} & & \multicolumn{4}{c}{Sum-of-Squares  } & \multicolumn{4}{|c}{Neural Barrier Function} \\ \cline{4-23}
  {Model} & {$|K|$} & $\mathcal{T}_{p} (s) $  &$\beta$ & $P_\safe$ &$\mathcal{T}_{0}(s)$ & 
  $\beta$ & $P_\safe$  & $\mathcal{I}$  & $\mathcal{T}_{o} (s) $& 
  $\beta$ & $P_\safe$  & $\mathcal{I}$  & $\mathcal{T}_{o} (s) $ & Deg & $\eta$ & $\beta$ & $P_\safe$ & $\mathcal{T}_{o} (s) $  & $\eta$ & $\beta$  &  $P_\safe$ & $\mathcal{T}_{o}$\\
  \hline 
  {Linear}  &  64 & 0.02 &  $8.4e^{-4}$  & 0.992 &  0.52
 & $8.4e^{-4}$&  0.992 & 2  &  0.04 &  $4.7e^{-3}$&  0.952 &  50 &   0.04  &4  & $2.4e^{-1}$ & $1.8e^{-2}$ &  0.582 & 0.014 & $7.1e^{-5}$ & $4.1e^{-2}$ & 0.585 & 3850.93 \\
2D  & 225 & 0.31 & $1.4e^{-4}$  & 0.998   & 164.60  & $1.4e^{-4}$ &  0.998 &  2 & 0.44 & $2.6e^{-3}$ & 0.973 & 50 & 0.20 &  8& $2.4e^{-1}$& $1.7e^{-2}$& 0.582 & 0.265 
 &$2.0e^{-3}$ &$5.8e^{-3}$  & 0.940 & 3991.47 \\ 
 \textit{Convex }  & 900  &  8.85 & $1.1e^{-4}$ & 0.999 & 1087.78  & $1.1e^{-4}$  & 0.999 & 2   & 17.93  & $1.0e^{-3}$ & 0.990  & 150 & 7.22 & 30 & $1.4e^{-2}$ &$7.6e^{-4}$  & 0.978  & 151.16   & $1.9e^{-3}$ & $3.7e^{-3}$ & 0.961 & 4025.67 \\
   & 2500  &   41.44 & $8.1e^{-5}$  & 0.999  & 2897.77  & $8.1e^{-5}$  & 0.999 & 2   & 88.45  &  $9.1e^{-4}$ & 0.998  & 175 & 52.78 & 36 & $7.0e^{-3}$
  & $5.9e^{-5}$   & 0.992  &    458.21 & $1.7e^{-3}$ &$2.2e^{-3}$ & 0.976 & 4085.65\\
\cline{3-16}
  \hline 
  {Linear}  & 900 & 5.04  & $5.1e^{-2}$  & 0.494  & 1197.99 
 & $5.1e^{-2}$  &  0.494 &  1 &  3.79  & $5.1e^{-2}$  & 0.494  & 50  &    3.52  &12  & $9.9e^{-1}$  & $1.0e^{-6}$ & 0.010  & 0.02 
 & 1.5$e^{-1}$ & 6.1$e^{-3}$& 0.792 & 3546.69
 \\
2D & 1225  & 8.20 & $2.0e^{-2}$ & 0.800  & 1389.78 & $2.0e^{-2}$ & 0.800  & 1 & 7.22 & $2.0e^{-2}$ & 0.800 &  50 & 6.64 & 20  & $9.9e^{-1}$ &  $2.3e^{-6}$ & 0.010 & 11.08 
& 1.5$e^{-1}$ & 5.4$e^{-3}$& 0.844&3579.58
\\ 
\textit{ Non-Convex} & 1444 & 9.18 & $7.9e^{-3}$ &  0.921 & 1545.45 & $7.9e^{-3}$& 0.921 &  1 & 11.65 &  $7.9e^{-3}$ & 0.921  & 55 & 10.12  & 24 & $9.2e^{-1}$ & $5.3e^{-3}$  & 0.023   & 37.89  &  1.4$e^{-1}$& 5.2$e^{-3}$& 0.855&3589.13  \\
   & 2926 & 47.98  & $7.2e^{-3}$ & 0.927  & 3161.56 &  $7.2e^{-3}$  & 0.927 & 2 &  98.36 &  $7.2e^{-3}$ & 0.927   & 115&  20.86   & 26 & $9.1e^{-1}$ & $5.6e^{-3}$  & 0.034   & 62.88 &  1.9$e^{-2}$ & 5.3$e^{-1}$ & 0.928 & 3599.85 \\
      & 5890 &  179.94 & $7.1e^{-3}$ & 0.929  & 8191.65 &  $7.1e^{-3}$  &  0.929& 3 & 458.44   & $7.1e^{-3}$   &  0.929  & 285 & 133.84 & 30 & $8.7e^{-1}$   & $4.7e^{-3}$ &  0.075 & 196.85 &1.8$e^{-2}$  &5.3$e^{-1}$ & 0.929& 3675.77\\
    & 11818 & 477.45  & - & -  & \texttt{TO}&  $6.4e^{-3}$  & 0.936 & 3 & 1875.49  &  $6.4e^{-3}$ & 0.936  & 445 & 842.67  & 34 & - & -  &  - & \texttt{OM} &1.7$e^{-2}$ &5.2$e^{-1}$ & 0.931 & 3744.23\\
        & 24336 &  987.65 & - & -  & \texttt{TO}& $6.2e^{-3}$  &  0.938  & 2 & 4441.55  &  $6.2e^{-3}$  & 0.938  & 595 & 3099.30   & 36 & - & -  &  - & \texttt{OM} &1.6$e^{-2}$ & 4.8$e^{-3}$& 0.936& 4234.56 \\
\cline{3-16}
 \hline
{Pendulum}  & 120 & 6.37 & 1.0$e^{-6}$& 1.00 & 0.51  & 1.1$e^{-4}$&  0.99  & 50& 5.84 &  1.1$e^{-3}$ & 0.989 & 15000 & 3.75  & 4 & 5.9$e^{-5}$ & 2.1$e^{-4}$ & 0.999 & 7.71  & 7.7$e^{-4}$ & 2.1$e^{-5}$ &0.999 & 4242.89 \\
 2D &   240 & 18.33 &  1.0$e^{-6}$ &  1.00 & 6.08 & 2.2$e^{-5}$& 1.00  &200   & 14.88 & 1.0$e^{-3}$& 0.990 & 20000 & 9.99  & 4 & 4.9$e^{-5}$ & 2.1$e^{-4}$ & 0.999 & 34.96 &7.6$e^{-4}$  & 2.1$e^{-5}$ & 0.999 & 4457.82 \\
 &  480 &  37.84 & 1.0$e^{-6}$ & 1.00 &29.39  & 2.0$e^{-6}$  &  1.00 &  300 &43.42 & 8.1$e^{-5}$   & 0.999  & 40000  & 17.88  & 4 & 4.8$e^{-5}$ & 2.0$e^{-4}$ & 0.999 & 187.60 & 5.8e$^{-4}$& 1.9$e^{-5}$ & 0.999 & 4675.12\\ \cline{3-16} 
  \hline
  {Unicycle}  &  1250 & 1103.42 & $2.5e^{-2}$ &  0.750 &  1000.19 & $2.5e^{-2}$  &  0.750& 200 & 26.37  & $2.5e^{-2}$ & 0.750 & 300 & 5.68 & 2  & $9.9e^{-1}$ & 1.0$e^{-6}$ & 0.00  & 3110.21   &\cellcolor{gray!25} & \cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25}\\
 4D &  1800 & 1756.25 & $2.5e^{-2}$ & 0.975  & 1719.58  &$2.5e^{-2}$& 0.975  & 200  & 92.26 & $2.5e^{-2}$   & 0.975 & 20000 & 25.78   & 4 & $9.9e^{-1}$ & 1.0$e^{-6}$ & 0.00  &   5451.19  &\cellcolor{gray!25} & \cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25}\\
 & 2400 & 2001.11
 & $2.1e^{-3}$  & 0.998 &  2548.56 &  $2.1e^{-3}$  & 0.998 & 200  & 145.45&  $2.1e^{-3}$  &0.998 &40000  & 55.59  & 6  & -& -& - & \texttt{OM} &\cellcolor{gray!25} & \cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25}\\
  \hline
   Quadrotor &  7865 & 80.80  & $2.3e^{-2}$ &0.770  & 9906.67 & $2.3e^{-2}$ & 0.770 & 450& 1174.49&  $2.3e^{-2}$ & 0.770   & 40000  & 2589.56&   2 & $8.8e^{-2}$ & $3.3e^{-2}$  & 0.584  & 0.20  &\cellcolor{gray!25} & \cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25}
   \\ 
6D  &  15625  & 160.61 & -& - & \texttt{TO}&  $9.9e^{-3}$ & 0.901 & 575 & 3788.98&  $9.9e^{-3}$ & 0.901  & 50000  & 3258.87 &   8   & $1.1e^{-3}$  &$9.9e^{-3}$  & 0.900 & 8628.58
  &\cellcolor{gray!25} & \cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25} \\ 
  \textit{Convex}   &  46656  & 458.59 &- &  - & \texttt{TO}&-  & - & -& \texttt{TO}&  $8.8e^{-3}$ & 0.912  & 120000  & 9542.75   & 12   & -  &-  &- &\texttt{OM} &\cellcolor{gray!25} & \cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25}\\  
  \hline
 Quadrotor &  15625&  188.10 &- & - &\texttt{TO}&$3.3e^{-2}$  & 0.670&595 & 3845.25  & $3.3e^{-2}$  & 0.670  & 55550 & 3478.31 &  4 & $9.9e^{-1}$& $1.0e^{-6}$ & 0.00  & 4.91 &\cellcolor{gray!25} & \cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25}\\ 
  6D &   31250& 395.59 &- & - &\texttt{TO}& $1.9e^{-2}$ & 0.810 & 615 & 9548.78 & $1.9e^{-2}$   & 0.810 & 89850 & 5878.28   &  8 & $9.9e^{-1}$& $1.0e^{-6}$ & 0.00  & 8715.54 &\cellcolor{gray!25} & \cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25} \\ 
 \textit{Non-Convex}  &  46656  & 506.99  &- &  - & \texttt{TO}&  -&- &- &\texttt{TO}&  $1.0e^{-2}$  & 0.900 & 121500  & 9789.54  & 12  &  - & - & -& \texttt{OM} &\cellcolor{gray!25} & \cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25}\\  
 \hline
   Quadrotor & 65536  & 845.44   & - &  -& \texttt{TO}& - & - & -& \texttt{TO}&$5.0e^{-2}$  & 0.500  & 198550  & 19377.90  & 2& $9.9e^{-1}$& $1.0e^{-6}$ & 0.00  & 14830.23 &\cellcolor{gray!25} & \cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25}\\ 
    8D & 128000 & 2530.74  &- & -& \texttt{TO}& - & - & - & \texttt{TO} & $4.4e^{-2}$  &  0.560 & 256700 & 39132.59 &   4  & - & - & - & \texttt{OM} &\cellcolor{gray!25} & \cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25}\\ 
 \hline
\bottomrule
\end{tabular}
%% ends scaling the table
}
% \text{$^{1}$ For linear systems that use Sum-of-Squares (\gls{sos}) optimization the state space is not partitioned.}
% \text{$^{2}$ The Sum-of-Squares (\gls{sos}) barrier synthesis is not based on optimization through transition probabilities.}
% \end{table*}
\end{sidewaystable*}


